KB-Plugin: A Plug-and-play Framework for Large Language Models to Induce Programs over Low-resourced Knowledge Bases

Program induction (PI) has become a promising paradigm for using knowledge bases (KBs) to help large language models (LLMs) answer complex knowledge-intensive questions. Nonetheless, PI typically relies on a large number of parallel question-program pairs to make the LLM aware of the schema of the given KB, and is thus challenging for many low-resourced KBs that lack annotated data. To this end, we propose KB-Plugin, a plug-and-play framework that enables LLMs to induce programs over any low-resourced KB. Firstly, KB-Plugin adopts self-supervised learning to encode the detailed schema information of a given KB into a pluggable module, namely schema plugin. Secondly, KB-Plugin utilizes abundant annotated data from a rich-resourced KB to train another pluggable module, namely PI plugin, which can help the LLM extract question-relevant schema information from the schema plugin of any KB and utilize this information to induce programs over this KB. Experiments on five heterogeneous KBQA datasets show that KB-Plugin achieves better or comparable performance with 25$\times$ smaller backbone LLM compared to SoTA PI methods for low-resourced KBs, and even approaches the performance of supervised methods. Our code and data are available at https://github.com/THU-KEG/KB-Plugin.

==> tables/ablation.tex <==
\begin{table}[t]
\centering
\scalebox{1.0}{
    \small
    \setlength{\tabcolsep}{2pt}
    \begin{tabular}{lccccc}
    \toprule
    \textbf{Method}              & \textbf{WebQSP} & \textbf{GraphQ} & \textbf{GrailQA} & \textbf{MetaQA} & \textbf{SoAyBC} \\\hline
    KB-Plugin                    & \textbf{57.2}   & \textbf{49.5}   & \textbf{62.7}    & \textbf{99.0}   & \textbf{84.3}      \\
    w/o schema plugin            & 41.0            & 42.8            & 57.5             &                 & 63.8               \\
    w/ m\_sc\textasciicircum{}S0 & 48.0            &                 & 51.0             & 90.1            & 61.0               \\ \bottomrule
    \end{tabular}
}
\label{main_freebase}
\end{table}

==> tables/function_examples.tex <==
\begin{table}[t]
  \centering
  \scalebox{0.85}{
    \small
    \setlength{\tabcolsep}{2pt}
    \begin{tabular}{ccccc}
    \toprule
        Function & \begin{tabular}{c} Argument \\ Type\end{tabular} & Argument & Description \\
        % \hline
        % $D(r)$ & $D(r) = \{c_i | (c_i, r, c_j) \in \mathcal{T}\}$, denoting the domain of relation $r$. \\
        \midrule
        \textit{Find} & entity & $\mathtt{FC\ Barcelona}$ & \begin{tabular}{c}
        Find the specific \\ KB entity \end{tabular}  \\
        \midrule
        \textit{Relate} & relation & $\mathtt{arena\ stadium}$ & \begin{tabular}{c} Find the entities that \\ hold a specific relation \\ with the given entity\end{tabular} \\
        \midrule
        \textit{FilterConcept} & concept & $\mathtt{sports\ facility}$ & \begin{tabular}{c} Find the entities that \\ belong to a specific \\ concept\end{tabular} \\
        \midrule
        \textit{And} & - & - & \begin{tabular}{c} Return the intersection \\ of two entity sets \end{tabular} \\
        % $R^{-}(c)$  & $R^{-}(c) = \{r | (c_i, r, c) \in \mathcal{T}\}$, denoting the relations whose ranges contain $c$. \\
        % \hline
        % $C(e)$ & $C(e) = \{ c | (e, \texttt{isA}, c) \in \mathcal{T} \}$, denoting the concepts of entity $e$. \\
    \bottomrule
    \end{tabular}
    }
    \caption{Function examples. - means empty.}
    \label{tab_func_example}
\end{table}
